Invariant Slot Attention: Object Discovery with Slot-Centric Reference Frames

Automatically discovering composable abstractions from raw perceptual data is a long-standing challenge in machine learning. Recent slot-based neural networks that learn about objects in a self-supervised manner have made exciting progress in this direction. However, they typically fall short at adequately capturing spatial symmetries present in the visual world, which leads to sample inefficiency, such as when entangling object appearance and pose. In this paper, we present a simple yet highly effective method for incorporating spatial symmetries via slot-centric reference frames. We incorporate equivariance to per-object pose transformations into the attention and generation mechanism of Slot Attention by translating, scaling, and rotating position encodings. These changes result in little computational overhead, are easy to implement, and can result in large gains in terms of data efficiency and overall improvements to object discovery. We evaluate our method on a wide range of synthetic object discovery benchmarks namely CLEVR, Tetrominoes, CLEVRTex, Objects Room and MultiShapeNet, and show promising improvements on the challenging real-world Waymo Open dataset.

==> csv/ablations.tex <==
method,test_miou,test_miou_sd,test_fg_ari,test_fg_ari_sd,test_mse,test_mse_sd,camo_miou,camo_miou_sd,camo_fg_ari,camo_fg_ari_sd,camo_mse,camo_mse_sd,ood_miou,ood_miou_sd,ood_fg_ari,ood_fg_ari_sd,ood_mse,ood_mse_sd
AST-Seg-B3-CT,79.6,0.5,\textbf{94.8},0.5,\textbf{139},7,73.1,0.7,\underline{87.3},3.8,\textbf{145},6,67.5,0.8,83.1,0.8,832,24
\isatsr,-,-,79.6,5.5,234.5,6.6,-,-,73.8,4.9,220.5,8.8,-,-,74.9,3.8,499.9,56.9
+ append,-,-,85.4,2.4,234.2,3.9,-,-,78.8,2.2,223.5,4.6,-,-,78.2,1.9,554.0,25.1
\isatsr (ResNet),-,-,93.3,0.7,185.9,6.4,-,-,87.0,1.7,206.1,10.0,-,-,\textbf{84.9},1.2,595.2,35.6
+ append,-,-,\underline{93.6},0.8,\underline{185.6},5.8,-,-,\textbf{87.5},0.9,\underline{201.1},6.9,-,-,\underline{84.8},0.7,647.1,24.6
- dec. only,-,-,93.4,1.0,200.4,6.6,-,-,87.2,1.7,223.5,5.3,-,-,83.9,1.6,614.4,49.7
- stop grad,-,-,73.4,10.5,392.6,116.5,-,-,62.8,10.3,388.2,81.2,-,-,67.5,8.0,621.9,62.8

==> csv/clevr_table_short.tex <==
method,fg_ari_mean,fg_ari_std,mse_mean,mse_std
AST-Seg-B3-CT,98.3,0.1,16,1
SA,98.8,0.2,13,2
\isat,99.0,0.2,11,2
\isats,98.9,0.2,11,1

==> csv/clevrtex_baselines.tex <==
method,test_miou,test_miou_sd,test_fg_ari,test_fg_ari_sd,test_mse,test_mse_sd,camo_miou,camo_miou_sd,camo_fg_ari,camo_fg_ari_sd,camo_mse,camo_mse_sd,ood_miou,ood_miou_sd,ood_fg_ari,ood_fg_ari_sd,ood_mse,ood_mse_sd
SPACE,9.1,3.5,17.5,4.1,298,80,8.7,3.5,10.6,2.1,251,61,6.9,3.3,12.7,3.4,387,66
DTI,33.8,1.3,79.9,1.4,438,22,27.5,1.6,72.9,1.9,377,17,32.6,1.1,73.7,1.0,590,4
Gen-V2,7.9,1.5,31.2,12.4,315,106,7.5,1.7,29.6,12.8,278,75,8.7,1.6,29.0,11.2,539,147
eMORL,12.6,2.4,45.0,7.8,318,43,11.6,2.1,42.3,7.2,269,31,13.2,2.6,43.1,9.3,471,51
AST-Seg-B3-CT,79.6,0.5,94.8,0.5,139,7,73.1,0.7,87.3,3.8,145,6,67.5,0.8,83.1,0.8,832,24

==> csv/clevrtex_resnet.tex <==
method,test_miou,test_miou_sd,test_fg_ari,test_fg_ari_sd,test_mse,test_mse_sd,camo_miou,camo_miou_sd,camo_fg_ari,camo_fg_ari_sd,camo_mse,camo_mse_sd,ood_miou,ood_miou_sd,ood_fg_ari,ood_fg_ari_sd,ood_mse,ood_mse_sd
ResNet SA,-,-,91.3,2.7,206.7,20.8,-,-,84.9,2.9,224.4,21.9,-,-,81.4,1.4,629.1,29.9
ResNet T-SA,-,-,87.4,6.6,197.1,27.0,-,-,79.0,5.9,217.6,24.5,-,-,78.6,4.9,548.1,21.3
ResNet TS-SA,-,-,92.9,0.4,176.9,3.4,-,-,86.2,0.8,196.3,7.1,-,-,84.4,0.8,578.3,22.5
ResNet TRS-SA,-,-,93.3,0.7,185.9,6.4,-,-,87.0,1.7,206.1,10.0,-,-,84.9,1.2,595.2,35.6
- dec. only,-,-,93.4,1.0,200.4,6.6,-,-,87.2,1.7,223.5,5.3,-,-,83.9,1.6,614.4,49.7
- stop grad,-,-,73.4,10.5,392.6,116.5,-,-,62.8,10.3,388.2,81.2,-,-,67.5,8.0,621.9,62.8
ResNet T-SA-Append,-,-,89.9,2.4,194.2,19.9,-,-,82.7,2.9,214.8,22.2,-,-,80.9,2.4,575.8,25.7
ResNet TS-SA-Append,-,-,92.6,1.3,180.0,11.2,-,-,86.0,1.5,197.3,8.9,-,-,83.8,1.1,606.1,57.5
ResNet TRS-SA-Append,-,-,93.6,0.8,185.6,5.8,-,-,87.5,0.9,201.1,6.9,-,-,84.8,0.7,647.1,24.6


==> csv/clevrtex_simplecnn.tex <==
method,test_miou,test_miou_sd,test_fg_ari,test_fg_ari_sd,test_mse,test_mse_sd,camo_miou,camo_miou_sd,camo_fg_ari,camo_fg_ari_sd,camo_mse,camo_mse_sd,ood_miou,ood_miou_sd,ood_fg_ari,ood_fg_ari_sd,ood_mse,ood_mse_sd
SimpleCNN SA,-,-,54.5,1.6,241.2,14.0,-,-,53.0,1.6,216.6,11.8,-,-,54.2,2.6,414.7,27.7
SimpleCNN T-SA,-,-,66.8,5.7,229.8,20.4,-,-,65.0,4.9,213.2,16.3,-,-,65.1,4.8,458.6,25.2
SimpleCNN TS-SA,-,-,78.8,3.9,223.8,6.5,-,-,72.9,3.5,210.9,6.2,-,-,73.2,3.1,480.6,32.6
SimpleCNN TRS-SA,-,-,79.6,5.5,234.5,6.6,-,-,73.8,4.9,220.5,8.8,-,-,74.9,3.8,499.9,56.9
SimpleCNN T-SA-Append,-,-,72.6,7.6,215.8,7.8,-,-,69.4,6.9,201.3,6.9,-,-,69.5,6.4,448.6,32.0
SimpleCNN TS-SA-Append,-,-,82.1,2.0,228.1,5.1,-,-,76.0,1.8,216.1,4.5,-,-,75.7,1.3,513.1,26.9
SimpleCNN TRS-SA-Append,-,-,85.4,2.4,234.2,3.9,-,-,78.8,2.2,223.5,4.6,-,-,78.2,1.9,554.0,25.1

==> csv/msne_all_objects.tex <==
method,data,fg_ari_mean,fg_ari_std,mse_mean,mse_std
SA,All,56.8,2.6,33,5
T-SA,All,71.2,3.5,29,3
TS-SA,All,69.8,1.1,27,1
TRS-SA,All,77.7,5.5,35,3

==> csv/msne_four_objects.tex <==
method,data,fg_ari_mean,fg_ari_std,mse_mean,mse_std
SA,Four objects,71.5,11.6,50,2
T-SA,Four objects,82.3,5.3,43,4
TS-SA,Four objects,86.5,1.1,41,3
TRS-SA,Four objects,80.7,6.4,51,6

==> csv/tetrominoes_left.tex <==
method,fg-ari,fg-ari-sd
SA,81.6,6.2
T-SA,96.3,3.6
- dec. only,92.3,2.4

==> csv/tetrominoes_samples.tex <==
num_samples,fg-ari_sa,fg-ari-sd_sa,fg-ari_t-sa,fg-ari-sd_t-sa,fg-ari_t-sa-dec,fg-ari-sd_t-sa-dec
64,64.1,7.0,72.9,6.3,64.6,5.7
128,75.1,5.6,87.9,6.7,80.7,4.4
256,80.5,6.4,91.4,6.3,81.4,3.5
512,90.4,4.0,97.3,4.1,86.2,2.3
1024,93.4,3.0,99.0,2.0,89.4,1.7

==> texsnippets/app_num_slots.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lll}
    \toprule
    Method      & Dataset           & Num. slots   & Appearance init.      & Reference frame init. \\
    \midrule

    SA          & Tetrominoes       & 4            & Learnable             & N/A                   \\
    \isat       & Tetrominoes       & 4            & Learnable             & Random                \\
\isat-dec. only & Tetrominoes       & 4            & Learnable             & Random                \\

    \midrule
    
    SA          & Objects room      & 11           & Learnable             & N/A                   \\
    \isat       & Objects room      & 11           & Learnable             & Learnable             \\
    \isats      & Objects room      & 11           & Learnable             & Learnable             \\
    \isatsr     & Objects room      & 11           & Learnable             & Learnable             \\
    
    \midrule
SA      & MultiShapeNet (All/Four objects) & 5     & Learnable             & N/A                   \\
\isat   & MultiShapeNet (All/Four objects) & 5     & Learnable             & Learnable             \\
\isats  & MultishapeNet (All/Four objects) & 5     & Learnable             & Learnable             \\
\isatsr & MultishapeNet (All/Four objects) & 5     & Learnable             & Learnable             \\
    
    \midrule
    SA          & CLEVR            & 11            & Learnable             & N/A                  \\
    \isat       & CLEVR            & 11            & Learnable             & Random               \\
    \isats      & CLEVR            & 11            & Learnable             & Random               \\
    \isatsr     & CLEVR            & 11            & Learnable             & Random               \\
    
    \midrule
   SA    (CNN)  & CLEVRTex         & 11            & Learnable             & N/A                  \\
   \isat (CNN)  & CLEVRTex         & 11            & Learnable             & Learnable            \\
   \isats(CNN)  & CLEVRTex         & 11            & Learnable             & Learnable            \\
  \isatsr(CNN)  & CLEVRTex         & 11            & Learnable             & Learnable            \\
 \isatsr(CNN) + Append  & CLEVRTex & 11            & Learnable             & Learnable            \\
 
    \midrule
   SA    (ResNet)  & CLEVRTex         & 11            & Learnable             & N/A                  \\
   \isat (ResNet)  & CLEVRTex         & 11            & Learnable             & Learnable            \\
   \isats(ResNet)  & CLEVRTex         & 11            & Learnable             & Learnable            \\
  \isatsr(ResNet)  & CLEVRTex         & 11            & Learnable             & Learnable            \\
 \isatsr(ResNet) + Append  & CLEVRTex & 11            & Learnable             & Learnable            \\
 \isatsr(ResNet) + Dec. only  & CLEVRTex & 11         & Learnable             & Learnable            \\
 \isatsr(ResNet) + Stop-grad  & CLEVRTex & 11         & Learnable             & Learnable            \\
 
    \midrule
    SA  (RGB)        & WaymoOpen           & 11            & Learnable             & N/A             \\
    \isats  (RGB)    & WaymoOpen           & 11            & Learnable             & Learnable       \\
    \isats-dec. only (RGB) & WaymoOpen       & 11            & Learnable             & Learnable       \\
    \isatsr (RGB) & WaymoOpen       & 11            & Learnable             & Learnable       \\
    SA (Depth) & WaymoOpen       & 11            & Learnable             & Learnable       \\
    \isat (Depth) & WaymoOpen       & 11            & Learnable             & Learnable       \\
    \isat-ABS (Depth) & WaymoOpen       & 11            & Learnable             & Learnable       \\
    \bottomrule
    \end{tabular}
\end{table}

==> texsnippets/clevrtex_mse_fig.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=0.7\linewidth]{figures/clevrtex_abl_mse.pdf}
  \vspace{-1.2em}
  \caption{CLEVRTex mean squared error: A box-plot comparing \isatsr and the decoder only ablation on reconstruction error.\tk{nit: different style than other box plots. also uses a lot of vertical space -- maybe a table would suffice here?}\am{I changed the style just now. From the table the conclusions about MSE being worse for the `Dec. only' ablation are not clear. Wdyt?}}
\label{fig:clevrtex:mse}
\end{figure}

==> texsnippets/msne_plt.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/msne_boxplt.pdf}
    \caption{\textbf{MultiShapeNet} FG-ARI results using 5 random seeds: Higher is better. For exact numbers see \cref{tab:msne}.}
    \label{fig:msne}
\end{figure}

==> texsnippets/objsrm_plt.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/objsrm_boxplt.pdf}
    \caption{\textbf{Objects Room} ARI with background segments included: Higher is better. We use 10 seeds per experiment. For exact numbers see \cref{tab:objects_room}.}
    \label{fig:objsrm}
\end{figure}
